A Dynamical View of the Question of Why

We address causal reasoning in multivariate time series data generated by stochastic processes. Existing approaches are largely restricted to static settings, ignoring the continuity and emission of variations across time. In contrast, we propose a learning paradigm that directly establishes causation between events in the course of time. We present two key lemmas to compute causal contributions and frame them as reinforcement learning problems. Our approach offers formal and computational tools for uncovering and quantifying causal relationships in diffusion processes, subsuming various important settings such as discrete-time Markov decision processes. Finally, in fairly intricate experiments and through sheer learning, our framework reveals and quantifies causal links, which otherwise seem inexplicable.

==> sections/background_full.tex <==
% \section{Background}
% The philosopher David Lewis, who founded ``counterfactual analysis of causation'' half a century ago, postulates that causation must always be transitive \cite{Lewis1973-ip}. He defines a causal chain as a finite sequence of events $a, b, c, \dots$ such that $b$ causally depends on $a$, $c$ causally depends on $b$, and so on. He advances his counterfactual analysis by asserting that an event is a cause of another event if and only if there is a causal chain from the first to the second (\cite{Lewis1973-ip}, p. 563). Moreover, Lewis emphasizes the importance of time and the temporal asymmetry of causation. In particular, he asserts that effects do not precede their causes, setting aside pathological cases like a time-machine or at the edge of a black-hole (see \cite{Lewis1979-rb}, p. 459). He summarized the discussion by three propositions \cite{Lewis1979-rb}:
% \begin{enumerate}
%     \item The relation of cause to effect consists in their being linked by a  causal chain;
%     \item Causal chain is a certain kind of chain of counterfactual dependencies; and 
%     \item The counterfactuals involved are to be taken under the standard resolution of vagueness.
% \end{enumerate}

 

% % \sg {So from this understanding of causation, the time of occurrence gives us the direction of a causal arrow, not essentially the presence or absence of one.}

% In Lewis discussions (re-emphasized later by Paul and others), we can pinpoint three core concepts: (1) time is an intrinsic part of the picture, (2) a chain of event must be definable and then forms the main ground for arguments about causation, and (3) such arguments adhere to the world, where laws (of physics) and facts are assumed to be directly considered (also see \cite{Lewis1979-rb}, p. 460). 

% We could see that all the points above have a direct connection to the mathematical concept of \textit{state-space modelling} and a (deterministic or stochastic) \textit{process} as the underlying dynamics of the world that evolves across time. If events are seen as a change of state or action variables, then a dynamical system represented by a process would directly render: (1) the intrinsic existence and inclusion of time, (2) ``chain of events'' and emission of events across time, and (3) the direct inclusion of laws of physics relevant to the problem at hand. 


% -----------

% Herein, we summarize those elegant classic arguments on the necessity for the inclusion of time in causal analysis through two basic axioms, which provide the foundation for our further definitions. Moreover, to allow for the probabilistic view of causality, we further add a third axiom. 

% A causal relationship contains two events: cause (event $A$) and effect (event $B$). In all logical arguments on causation, the following axioms are true. %In order to clearly set the problem, we build our theory on three core axioms. 

% \begin{enumerate}[i.]
%     \item Causality necessitates time: a causal relationship is realisable solely along the time axis.
%     \item Cause necessarily happens before effect and the relationship is unidirectional from cause to effect.
%     \item A causal relationship may imply neither necessity nor sufficiency. 
%     % \sg{How would we view such a condition w.r.t to a causal graph?}
% \end{enumerate}

% These axioms sets the ground for a natural view on the concept of causality. Notably, (i) requires that an event must be associated with a point or an interval in time; otherwise, no causal argument can possibly be made about that event being the cause or effect of any other event. For example, this axiom rejects the cases where one argues about causality between two random variables without any reference to the time. Remark that one may argue about correlation or dependency between ``any'' two random variables with no reference to time. \textcolor{red}{When arguing about causation, the time dependency often becomes implicit in the arguments (e.g., in causal graphs), but it may be a source of confusion; hence, we seek a formulation that inherently includes time; e.g., a stochastic dynamic process.} Next, (i) and (ii) necessitate that ``$A$ causes $B$'' implies ``$B$ \textit{cannot} cause $A$''; hence, causality necessitates a different characterization than merely correlation or dependency. The well-known statement that causality is not correlation would be a consequence of the first two axioms. Furthermore, (iii) necessitates that, in general, a causal relationship requires probabilistic views and non-binary measures. For example, if ``$A$ causes $B$'' and if $A$ does not happen, then in general, one cannot conclude $B$ necessarily will not happen. By the same token, if $A$ happens, it may not necessarily imply $B$ will also happen. \textcolor{red}{In other words, an event may partially contribute in the occurrence of another event in the future, although the case that $A$ is a necessary and sufficient cause for $B$ is a possibility.} This third axiom also implies that a well-defined causal relationship requires to identify the extent to which $A$ causes $B$. That is, in general, reasoning about causality requires a \textit{measure}; more on which will be said in the Section XXX.
% %To see the need for Axiom iii, consider the following example. Tom, Mike, and Ben moved the sofa. Tom is more strong than Mike and Ben together, and he held one side of the sofa, while the other side is held with equal share by both Mike and Ben. What did cause the sofa to move? The answer is clearly the effort of all the three boys; non of whom could have moved the sofa alone, that is, each individual contribution is not sufficient. Say Alex is also standing in the room and he is as strong as Tom. If Alex would have replaced Mike and Ben, they could still move the sofa. Hence, Mike and Ben's contribution was not necessary; they were only partially sufficient. The causation in an example of this sort is embraced by axiom iii. 

% \begin{figure}[t]
%     \centering
%     \includegraphics[width=3in]{images/process.pdf}
%     \caption{A sample path of a diffusion process with two state variables is shown. Change of $X_1$ from $t_1$ to $t_2$ is defined as event $A$ (blue), and change of $X_2$ from $t_3$ to $t_4$ is defined as $B$ (red); hence, $X_1$ and $X_2$ are their corresponding ruling variables. The question is whether or not $A$ is a cause for $B$.}
%     \label{fig:diffusion}
% \end{figure}

% % Our plan is to frame the problem of causality discovery in terms of a stochastic process. We are particularly interested in \textit{stochastic decision processes} to also account for actions taken by the agents (human or otherwise). \textcolor{red}{Hence, we first cite basic definitions in probabilistic terms from classic sources and then extend them to the generic case, in which actions exist.} In so doing we will introduce two core concepts of \textit{grit} and \textit{reachablity}, and ground our definitions based upon them. We next present various theoretical results, which provide analytical/computational tools to discover causal relations and answer the question of why. Lastly, we provide formal results to transform the system-theoretic notions of grit and reachability into two particular RL problems. This last step completes the loop and enables answering the question of why directly from data. 

% % \subsection{Principles}

% % Page 573 of causation (1973) states that a causal dependence require two counterfactuals: $B$ causally depends on $A$ and $\neg B$ causally depends on $\neg A$.

% ---------------

% The probabilistic version of the analysis (\cite{Lewis1986-LEWPTC}, pp. 175–84, also described in \cite{Paul1998-time}) states the following:
% \begin{quote}
%     The effect $B$ depends probabilistically on a cause $A$ if and only if, given $A$, there is a chance $x$ of $B$’s occurring, and if $A$ were not to occur, there would be a chance $y$ of $B$’s occurring, where $x$ is much greater than $y$.
% \end{quote}

% This definition suffers from two basic issues. First, it dismisses the possibility of \textit{actions}, i.e., external inputs to the environment/system which are adjustable. Indeed, the probability of $B$ is not a fix number and it depends on the courses of actions after $A$ and until $B$'s occurrence. Second, as also noted by Pearl, the phrase ``if $A$ were not to occur'' is not well-defined since various things may occur in the absence of $A$, and it is unsettled which ones are acceptable.


% In an appropriate analysis, \textcolor{blue}{Paul postulates that a causal link includes a chain of (probabilistic) events from cause to the effect.} We formalize this notion by adhering to a stochastic decision process that governs the so-called chain of event of any kind. In other words, there is an underlying stochastic decision process, which comprises both state evolution of the world and all the physical interventions between $A$ and $B$. We remark that if $A$ causes $B$ then under the most pessimistic version of such a chain of events, still $x$ must be greater than $y$. \textcolor{blue}{Hence, we set $x$ to be the \textit{minimum} probability of $B$'s happening if $A$ happens; the ``minimum'' here takes into account the effect of other controllable parts of the environment from when $A$ is done until $B$ occurs.} \sg {Taking stochastic decision process to govern the chain of events provides enough justification to why we take minimum probability.}
% We should next examine whether a candidate event $A$ would increase $x$ and how much.

% % \paragraph{Remark.} We note that causality is more than correlation with past; that is, consideration of time is necessary but it not all to be worried about. First, mere correlation (but no causation) with past events can still exists. For example, rains starts, a few seconds later, Sarah who stands on top of a high hill opens her umbrella, a few seconds later rain drops reach down the hill and make the ground wet. Sarah's umbrella is clearly not a cause of the ground getting wet, while the two events are correlated. Second, causation is more than knowing the state in a single point in time; it is rather about how the state evolves to shape the effect. That is, mere prediction of future states \textit{does not} by itself answer the question of why; rather, we need to truly argue about whether \textit{an event} increases the minimum probability of the effect. Finally, if the world's dynamics is Markovian, then history of more than one stopping time is irrelevant and everything is encapsulated in the immediate past. 
% %However, the actual cause of an event in the current time can happen several time steps earlier, even if the dynamics is Markovian. 
% It is important to note that Markovian property of the state does not refute the cause event to reside in many time steps earlier. That is because a variation in a state component $X_{1}$ from say $t_0$ to $t_1$ will propagate in itself as well as other components (according to the dynamics) as time elapses till the effect occurs. As such, even if the state is Markovian, the root cause still is the original change of $X_1$. The main challenge which we will address in this paper is to characterize this causal link from past to future. In a related note, we also require the theory to cover stochasticity in the sense that repeating a scenario can produce a different trajectory of state. Hence, our measures must encompass the \textit{expected} evolution of the state from cause to effect.

% % That is because the value of immediate past state (even if it is self-contained and the current state is only a function of immediate past) still depends on, for example, the initial conditions as well as the random path from the initial conditions. Changing the initial conditions or taking a different sample trajectory can change our immediate past. We particularly shape our theory in a way to inherently address both counts. 


% \newpage

